Cascaded Self-Evaluation Augmented Training for Lightweight Multimodal LLMs

Efficient Multimodal Large Language Models (EMLLMs) can improve performance through Chain-of-Thought (CoT) reasoning, but they have poor self-evaluation capabilities during the CoT reasoning process. This is due to their tendency to simplify the reasoning process and the degradation of self-evaluation ability during downstream task fine-tuning. To address this, we intuitively propose \textit{Self-Evaluation Augmented Training (SEAT)}, which uses more powerful EMLLMs to evaluate CoT reasoning data. The evaluation data is then used to train EMLLMs. However, due to the difficulties EMLLMs face with processing long token input-output sequences, and the degradation of self-evaluation ability as a basis for CoT reasoning, the SEAT method is not fully adapted. Therefore, we further propose \textit{Cascaded Self-Evaluation Augmented Training (Cas-SEAT)}, which converts long prompts into cascaded short prompts, each focusing on a specific task. Additionally, we mix CoT reasoning and self-evaluation data to preserve its CoT reasoning ability while enhancing the self-evaluation capability of EMLLMs. We also conduct \textit{Double-level Data Filtering (DDF)}, which includes source data filtering and labeled data filtering, using both manual selection and MLLMs for filtering. Cas-SEAT and DDF work together to improve the performance of EMLLMs. Experiments show that Cas-SEAT achieves an average improvement of 22.16% across multiple datasets, and DDF significantly reduces the resource consumption of training

==> table/main_table_mathv_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccccc}
 & \multicolumn{6}{c}{\textbf{Math-V}} \\
\multirow{-2}{*}{\textbf{Extra   Data}} & All & Level1 & Level2 & Level3 & Level4 & Level5 \\
\multicolumn{7}{c}{\textit{Open-Source Models   Inference}} \\
Base & 0.0526 & 0.0800 & 0.0690 & 0.0364 & 0.0444 & 0.0299 \\
Finetune & 0.1743 & 0.2075 & 0.1951 & 0.0893 & 0.1778 & 0.1912 \\
CoT & 0.1414 & 0.2075 & 0.1951 & 0.0893 & 0.1778 & 0.1912 \\
SEAT & 0.0757 & 0.1400 & 0.0690 & 0.0364 & 0.0444 & 0.0896 \\
Cas-SEAT & 0.1711 & 0.2075 &  0.1951 &  0.0893 & 0.1778 &  0.2059 \\
\multicolumn{7}{c}{\textit{Open-Source Models   Self-Evaluation}} \\
Base & 0.0757 & 0.1509 & 0.1098 & 0.0714 & 0.2222 & 0.1765 \\
Finetune & {\ul 0.1776} & 0.2075 & 0.1951 & 0.0893 & 0.1778 & 0.2059 \\
CoT & 0.1447 & 0.1321 & 0.1341 & 0.2321 & 0.1778 & 0.1912 \\
SEAT & 0.1447 & 0.1509 & 0.1098 & 0.0714 &  0.2222 & 0.1912 \\
\rowcolor[HTML]{DDEBF7} 
\textbf{Cas-SEAT} & \textbf{0.2763} & \textbf{0.2642} & \textbf{0.2439} & \textbf{0.2500} & \textbf{0.3111} & \textbf{0.3235} \\
\cellcolor[HTML]{EDEDED}\textit{Improve} & 55.57\% & 27.33\% & 25.01\% & 7.71\% & 40.01\% & 57.12\%
\end{tabular}
}
\vspace{-0.1cm}
\caption{Comparison of Cas-SEAT and the Baseline on Math-V Dataset}
\label{tab:main_mathv}
\vspace{-0.1cm}
\end{table}

==> table/pseudo_code.tex <==
\begin{algorithm}[!h]
\begin{flushleft}
  \caption{BELLS: Bidirectional Enhanced Learning for Large Language Model and Small Recommendation Model}
    
\textbf{Module 1:}~\colorbox{gray!30}{$\rhd$~\emph{Item to Semantic}}
    \resizebox{0.46\textwidth}{!}{
    \begin{tcolorbox}[sharp corners, colframe=gray!80!white, colback=white, boxrule=0.5mm, left=0pt, right=0pt, top=0pt, bottom=0pt, boxsep=5pt]
    % \begin{algorithmic}[1]
    \begin{algorithmic}
    \State \textbf{Target}: Item Sequence $s_v$ $\mapsto$ Semantic Sequence $s_c$ 
    \State \textbf{Input}: Item Sequence $s_v$
    \State \textbf{Output}: Semantic Sequence $s_c$
    \end{algorithmic}
    \end{tcolorbox}
    }

% \BlankLine
\textbf{Module 2:}~\colorbox{gray!30}{$\rhd$~\emph{Semantic Parameter Generation}}
\resizebox{0.46\textwidth}{!}{
    \begin{tcolorbox}[sharp corners, colframe=gray!80!white, colback=white, boxrule=0.5mm, left=0pt, right=0pt, top=0pt, bottom=0pt, boxsep=5pt]
    % \begin{algorithmic}[1]
    \begin{algorithmic}
    \State \textbf{Target}: Semantic Sequence $s_c$ $\mapsto$ Semantic Parameter Generator $\mathcal{M}_c$ and Semantic Encoder $E_c$ 
    \State \textbf{Input}: Semantic Sequence $s_c$
    \State \textbf{Output}: (Parameter $\Theta_d$), Prediction $\hat{y}$
    \end{algorithmic}
    \end{tcolorbox}
    }

% \BlankLine
\textbf{Module 3:}~\colorbox{gray!30}{$\rhd$~\emph{Semantic Metacode Learning}}
\resizebox{0.46\textwidth}{!}{
    \begin{tcolorbox}[sharp corners, colframe=gray!80!white, colback=white, boxrule=0.5mm, left=0pt, right=0pt, top=0pt, bottom=0pt, boxsep=5pt]
    % \begin{algorithmic}[1]
    \begin{algorithmic}
    \State \textbf{Target}: Item Sequence $s_v$, Semantic Sequence $s_c$ $\mapsto$ Item Parameter Generator $\mathcal{M}_v$, Item Encoder $E_v$, Semantic Parameter Generator $\mathcal{M}_c$, and Semantic Encoder $E_c$ 
    \State \textbf{Input}: Item Sequence $s_v$, Semantic Sequence $s_c$
    \State \textbf{Output}: (Parameter $\Theta_d$), Prediction $\hat{y}$
    \end{algorithmic}
    \end{tcolorbox}
    }

% \BlankLine
\textbf{Module 4:}~\colorbox{gray!30}{$\rhd$~\emph{Semantic Codebook Learning}}
\resizebox{0.46\textwidth}{!}{
    \begin{tcolorbox}[sharp corners, colframe=gray!80!white, colback=white, boxrule=0.5mm, left=0pt, right=0pt, top=0pt, bottom=0pt, boxsep=5pt]
    % \begin{algorithmic}[1]
    \begin{algorithmic}
    \State \textbf{Target}: Item Sequence $s_v$, Semantic Sequence $s_c$, Semantic Encoder $E_c$ $\mapsto$ Codebook $D$
    \State \textbf{Input}: Item Sequence $s_v$, Semantic Sequence $s_c$, (Semantic Encoder $E_c$)
    \State \textbf{Output}: (Parameter $\Theta_d$), Prediction $\hat{y}$
    \end{algorithmic}
    \end{tcolorbox}
    }

% \BlankLine
\textbf{Overview:}~\colorbox{gray!30}{$\rhd$~\emph{Training Procedure}}\\
    \textbf{Input}: Item Sequence $s_v$, Semantic Sequence $s_c$. \\
    \textbf{Output}: (Parameters $\Theta_d$), Prediction $\hat{y}$.\\
    \textbf{Initialization}: Randomly initialize the models $\mathcal{M}$, $\mathcal{M}_c$, $\mathcal{M}_v$ with parameters $\Theta_s$, $\Theta_c$, $\Theta_v$ respectively. \\
    Item Sequence $s_v$  $\mapsto$ Semantic Sequence $s_c$\\
    \Repeat {Convergence}{
     \If{Semantic Parameter Generator $\mathcal{M}_c$ and Semantic Encoder $E_c$ have not yet been well-trained} 
     {
           Train as follows (see Eq.12 for the details),\\
           $\mathop{\rm min}_{\Theta_s, \Theta_c, \Theta_v}\mathcal{L} = \sum\nolimits_{u, v, s_c, y\in\mathcal{D}}l_{\text{CE}}(y, \hat{y})$ \\
           }
          }
  \textbf{Initialization}: Initialize the Codebook $D$ via pretrained Semantic Encoder $E_c$\\
  \Repeat {Convergence}{
  \If{Semantic Parameter Generator $\mathcal{M}_c$ and Semantic Encoder $E_c$ have not yet been well-trained} 
    {
        Train as follows (see Eq.13 for the details),\\
        $\mathop{\rm min}_{\Theta_s, \Theta_c, \Theta_v}\mathcal{L} = \sum\nolimits_{u, v, s_c, y\in\mathcal{D}}l_{\text{CE}}(y, \hat{y}) + \lambda l_{\text{MSE}}(\mathbf{E}_v, \mathbf{E}_v'), $\\
    }
    }
    \Return{$\mathcal{M}_c$, $\mathcal{M}_v$, $D$}.\\
    % }
\label{alg:pseudo_code}
\end{flushleft}
\end{algorithm}


==> tex/6limitation.tex <==
\section*{Limitation}

% Dynamic role allocation mechanism proposed by our Bidirectional Enhanced Learning framework (\method{}) is effective, but costs more than only training the LLMs and SRMs. Although it is not so important in the most cases.
% Potential limitations may include a small amount of resource consumption. The method is designed specifically for EMLLMs, and it may not currently be the optimal solution for larger MLLMs.
While we optimize the cost of Cas-SEAT for resource-constrained settings, the training still involves additional data annotation and model retraining steps. This overhead could be further minimized, particularly in environments where computational resources are extremely limited. Future work could explore even more efficient methods of training or alternative ways to incorporate self-evaluation without adding significant computational burden.

==> tex/acknowledgement.tex <==
\section*{ACKNOWLEDGEMENTS}
\begin{sloppypar}
% \noindent \textbf{Acknowledgement}
This work was supported in part by National Key Research and Development Program of China (2022YFC3340900), National Natural Science Foundation of China (U20A20387, No. 62006207, No. 62037001), Project by Shanghai AI Laboratory (P22KS00111), Program of Zhejiang Province Science and Technology (2022C01044), the StarryNight Science Fund of Zhejiang University Shanghai Institute for Advanced Study (SN-ZJU-SIAS-0010), Fundamental Research Funds for the Central Universities (226-2022-00142, 226-2022-00051), the National Research Foundation, Singapore under its Emerging Areas Research Projects (EARP) Funding Initiative. 
% Any opinions, findings and conclusions or recommendations expressed in this material are those of the author(s) and do not reflect the views of National Research Foundation, Singapore.
% \vspace{-0.6cm}
\end{sloppypar}
